RAGME: Retrieval Augmented Video Generation for Enhanced Motion Realism

Video generation is experiencing rapid growth, driven by advances in diffusion models and the development of better and larger datasets. However, producing high-quality videos remains challenging due to the high-dimensional data and the complexity of the task. Recent efforts have primarily focused on enhancing visual quality and addressing temporal inconsistencies, such as flickering. Despite progress in these areas, the generated videos often fall short in terms of motion complexity and physical plausibility, with many outputs either appearing static or exhibiting unrealistic motion. In this work, we propose a framework to improve the realism of motion in generated videos, exploring a complementary direction to much of the existing literature. Specifically, we advocate for the incorporation of a retrieval mechanism during the generation phase. The retrieved videos act as grounding signals, providing the model with demonstrations of how the objects move. Our pipeline is designed to apply to any text-to-video diffusion model, conditioning a pretrained model on the retrieved samples with minimal fine-tuning. We demonstrate the superiority of our approach through established metrics, recently proposed benchmarks, and qualitative results, and we highlight additional applications of the framework.

==> tables/complexity.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|cc|cc}
    \toprule
    \textbf{Method} &  FLOPS $(\downarrow)$ &  Latency \\
    \midrule
    ZeroScope &  1280  &    0.922 &             0.962010 &                0.984180 \\
    ZeroScope + FreeInit  & 0.0  &       0.922 &             0.962010 &      0.984180 \\
    DDIM Inversion
    ZeroScope + RInit &   0.0  &    0.952 &             0.960735 &                0.984552 \\
    \rowcolor{cyan} \methodname &  618  &       0.976 &             0.913018 &                0.970199 \\
    \bottomrule
    \end{tabular}}
    \caption{Computational complexity of different methods.}
    \label{tab:complexity}
\end{table}
    


==> tables/noise_init.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|cc|cc}
    \toprule
    \textbf{Method} &  FVD $(\downarrow)$ &  FID $(\downarrow)$ & DINO-S $(\downarrow)$ &  LPIPS $(\uparrow)$  \\
    \midrule
    Single Latent \\
    DDIM Inversion \\
    Avg Latents \\
    \rowcolor{cyan} \methodname &  618  &       0.976 &             0.913018 &                0.970199 \\
    \bottomrule
    \end{tabular}}
    \caption{}
    \label{tab:nosie_init}
\end{table}
    


==> tables/quantiative.tex <==
\begin{table*}[!hbt]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}}& \multicolumn{2}{c|}{\textbf{Video Quality}} & \multicolumn{2}{c|}{\textbf{Temporal Consistency}} & \multicolumn{3}
        {c|}{\textbf{Image Alignment}} & \multicolumn{1}{c}{\textbf{Bckg. Preservation}} \\ \cmidrule{2-9}
        \multicolumn{1}{c}{} & DOVER \myarrowup & \multicolumn{1}{c|}{FVD\myarrowdown} & WE\myarrowdown & \multicolumn{1}{c|}{CLIP-T \myarrowup} & CLIP-S \myarrowup & DINO-S \myarrowup & \multicolumn{1}{c|}{LPIPS \myarrowdown} & L1 \myarrowdown \\ 
        \midrule

        PAIR Diffusion \cite{goel2023pair} & 0.602 &  24.32 & 19.6 & 0.904 & 0.552 & \textbf{0.36} & \textbf{0.71 } & \textbf{0.029} \\
        FILM \cite{reda2022film} & 0.643 & 19.85 & 8.9 & 0.956 & 0.546 & 0.33 & 0.76 & 0.035 \\
        TokenFlow \cite{geyer2023tokenflow} & \textbf{0.675} & 18.67 & \textbf{6.1} & \textbf{0.957}  & 0.501 & 0.29 & 0.81 & 0.101 \\
        Pix2Video \cite{ceylan2023pix2video} & 0.668 & 20.60 & 7.4 & 0.954 & 0.49 & 0.33 & 0.76 & 0.096 \\ 
        \rowcolor{yellow} \methodname & 0.672 & \textbf{16.54} & 9.8 &  0.955 & \textbf{0.567} & \textbf{0.36} & 0.73 & 0.036 \\
        \bottomrule
    \end{tabular}}
    \caption{Quantitative results for the task of Image Driven Appearance Editing. FVD and WE have been rescaled by a factor of $10^2$, $10^{-3}$.}
    \label{tab:metrics_appearnace_editing}
\end{table*}

==> tables/vbench_all.tex <==
\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{llrrrrrrrrrrrrrrrrrrr}
 method & aesthetic quality & appearance style & background consistency & color & dynamic degree & human action & imaging quality & motion smoothness & multiple objects & object class & overall consistency & scene & spatial relationship & subject consistency & temporal flickering & temporal style & tot_final_score & tot_quality_score & tot_semantic_score \\
ZeroScope & 0.530 & 0.235 & 0.984 & 0.922 & 0.367 & 0.922 & 0.663 & 0.985 & 0.417 & 0.841 & 0.257 & 0.443 & 0.499 & 0.962 & 0.986 & 0.259 & 0.785 & 0.804 & 0.709 \\
FreeInit & 0.542 & 0.229 & 0.990 & 0.915 & 0.242 & 0.912 & 0.641 & 0.988 & 0.441 & 0.876 & 0.255 & 0.424 & 0.379 & 0.978 & 0.994 & 0.252 & 0.781 & 0.803 & 0.693 \\
RagInit & 0.550 & 0.231 & 0.985 & 0.904 & 0.467 & 0.952 & 0.631 & 0.985 & 0.433 & 0.895 & 0.265 & 0.513 & 0.475 & 0.961 & 0.990 & 0.259 & 0.795 & 0.812 & 0.726 \\
\methodname & 0.519 & 0.228 & 0.972 & 0.865 & 0.742 & 0.976 & 0.574 & 0.968 & 0.389 & 0.893 & 0.267 & 0.492 & 0.341 & 0.911 & 0.982 & 0.255 & 0.776 & 0.795 & 0.699 \\
\end{tabular}}
\end{table}

